Improving HEVC Encoding of Rendered Video Data Using True Motion Information

This paper shows that motion vectors representing the true motion of an object in a scene can be exploited to improve the encoding process of computer generated video sequences. Therefore, a set of sequences is presented for which the true motion vectors of the corresponding objects were generated on a per-pixel basis during the rendering process. In addition to conventional motion estimation methods, it is proposed to exploit the computer generated motion vectors to enhance the ratedistortion performance. To this end, a motion vector mapping method including disocclusion handling is presented. It is shown that mean rate savings of 3.78% can be achieved.

==> gfx/RD_Rect80_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA data2}%
\psfrag{009}[cl][cl]{\matlabtextA dassssssta1}%
\psfrag{010}[bc][bc]{\matlabtextA PSNR [dB]}%
\psfrag{011}[tc][tc]{\matlabtextA File size [Bits]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $10^{5}$}%
\psfrag{001}[ct][ct]{\matlabtextA $10^{6}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{002}[rc][rc]{\matlabtextA $42$}%
\psfrag{003}[rc][rc]{\matlabtextA $44$}%
\psfrag{004}[rc][rc]{\matlabtextA $46$}%
\psfrag{005}[rc][rc]{\matlabtextA $48$}%
\psfrag{006}[rc][rc]{\matlabtextA $50$}%
\psfrag{007}[rc][rc]{\matlabtextA $52$}%
%
%% </ytick>

==> gfx/RD_time_hexaCIF_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{021}[cl][cl]{\matlabtextA data2}%
\psfrag{022}[cl][cl]{\matlabtextA datsssssssssa1}%
\psfrag{023}[bc][bc]{\matlabtextA PSNR [dB]}%
\psfrag{024}[tc][tc]{\matlabtextA Encoding Times [s]}%
\psfrag{025}[bc][bc]{\matlabtextA PSNR [dB]}%
\psfrag{026}[tc][tc]{\matlabtextA File size [Bits]}%
%
%% </text>
%
%% <xscale>
%
\psfrag{010}[tc][tc]{\matlabtextA $\times10^{4}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $60$}%
\psfrag{001}[ct][ct]{\matlabtextA $80$}%
\psfrag{002}[ct][ct]{\matlabtextA $100$}%
\psfrag{003}[ct][ct]{\matlabtextA $120$}%
\psfrag{011}[ct][ct]{\matlabtextA $0$}%
\psfrag{012}[ct][ct]{\matlabtextA $5$}%
\psfrag{013}[ct][ct]{\matlabtextA $10$}%
\psfrag{014}[ct][ct]{\matlabtextA $15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextA $36$}%
\psfrag{005}[rc][rc]{\matlabtextA $38$}%
\psfrag{006}[rc][rc]{\matlabtextA $40$}%
\psfrag{007}[rc][rc]{\matlabtextA $42$}%
\psfrag{008}[rc][rc]{\matlabtextA $44$}%
\psfrag{009}[rc][rc]{\matlabtextA $46$}%
\psfrag{015}[rc][rc]{\matlabtextA $36$}%
\psfrag{016}[rc][rc]{\matlabtextA $38$}%
\psfrag{017}[rc][rc]{\matlabtextA $40$}%
\psfrag{018}[rc][rc]{\matlabtextA $42$}%
\psfrag{019}[rc][rc]{\matlabtextA $44$}%
\psfrag{020}[rc][rc]{\matlabtextA $46$}%
%
%% </ytick>

==> gfx/RD_time_hexaHD_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{024}[cl][cl]{\matlabtextA data2}%
\psfrag{025}[cl][cl]{\matlabtextA datdddddddddda1}%
\psfrag{026}[bc][bc]{\matlabtextA PSNR [dB]}%
\psfrag{027}[tc][tc]{\matlabtextA Encoding Times [s]}%
\psfrag{028}[bc][bc]{\matlabtextA PSNR [dB]}%
\psfrag{029}[tc][tc]{\matlabtextA File size [Bits]}%
%
%% </text>
%
%% <xscale>
%
\psfrag{011}[tc][tc]{\matlabtextA $\times10^{5}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1000$}%
\psfrag{001}[ct][ct]{\matlabtextA $1500$}%
\psfrag{002}[ct][ct]{\matlabtextA $2000$}%
\psfrag{003}[ct][ct]{\matlabtextA $2500$}%
\psfrag{012}[ct][ct]{\matlabtextA $0$}%
\psfrag{013}[ct][ct]{\matlabtextA $2$}%
\psfrag{014}[ct][ct]{\matlabtextA $4$}%
\psfrag{015}[ct][ct]{\matlabtextA $6$}%
\psfrag{016}[ct][ct]{\matlabtextA $8$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextA $41$}%
\psfrag{005}[rc][rc]{\matlabtextA $42$}%
\psfrag{006}[rc][rc]{\matlabtextA $43$}%
\psfrag{007}[rc][rc]{\matlabtextA $44$}%
\psfrag{008}[rc][rc]{\matlabtextA $45$}%
\psfrag{009}[rc][rc]{\matlabtextA $46$}%
\psfrag{010}[rc][rc]{\matlabtextA $47$}%
\psfrag{017}[rc][rc]{\matlabtextA $41$}%
\psfrag{018}[rc][rc]{\matlabtextA $42$}%
\psfrag{019}[rc][rc]{\matlabtextA $43$}%
\psfrag{020}[rc][rc]{\matlabtextA $44$}%
\psfrag{021}[rc][rc]{\matlabtextA $45$}%
\psfrag{022}[rc][rc]{\matlabtextA $46$}%
\psfrag{023}[rc][rc]{\matlabtextA $47$}%
%
%% </ytick>

==> gfx/carshow_BD_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{017}[cl][cl]{\matlabtextA data4}%
\psfrag{018}[cl][cl]{\matlabtextA data3}%
\psfrag{019}[cl][cl]{\matlabtextA data2}%
\psfrag{020}[cl][cl]{\matlabtextA ddddddddata1}%
\psfrag{021}[bc][bc]{\matlabtextA PSNR [dB]}%
\psfrag{022}[tc][tc]{\matlabtextA File size [MBits]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $0.5$}%
\psfrag{002}[ct][ct]{\matlabtextA $1$}%
\psfrag{003}[ct][ct]{\matlabtextA $1.5$}%
\psfrag{004}[ct][ct]{\matlabtextA $2$}%
\psfrag{005}[ct][ct]{\matlabtextA $1$}%
\psfrag{006}[ct][ct]{\matlabtextA $1.2$}%
\psfrag{007}[ct][ct]{\matlabtextA $1.4$}%
\psfrag{008}[ct][ct]{\matlabtextA $1.6$}%
\psfrag{009}[ct][ct]{\matlabtextA $1.8$}%
\psfrag{010}[ct][ct]{\matlabtextA $2.0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextA $42$}%
\psfrag{012}[rc][rc]{\matlabtextA $44$}%
\psfrag{013}[rc][rc]{\matlabtextA $46$}%
\psfrag{014}[rc][rc]{\matlabtextA $48$}%
\psfrag{015}[rc][rc]{\matlabtextA $50$}%
\psfrag{016}[rc][rc]{\matlabtextA $52$}%
%
%% </ytick>

==> gfx/carshow_time_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA data4}%
\psfrag{013}[cl][cl]{\matlabtextA data3}%
\psfrag{014}[cl][cl]{\matlabtextA data2}%
\psfrag{015}[cl][cl]{\matlabtextA dssssssata1}%
\psfrag{016}[bc][bc]{\matlabtextA PSNR [dB]}%
\psfrag{017}[tc][tc]{\matlabtextA Encoding Times [s]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $2500$}%
\psfrag{001}[ct][ct]{\matlabtextA $3000$}%
\psfrag{002}[ct][ct]{\matlabtextA $3500$}%
\psfrag{003}[ct][ct]{\matlabtextA $4000$}%
\psfrag{004}[ct][ct]{\matlabtextA $4500$}%
\psfrag{005}[ct][ct]{\matlabtextA $5000$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $42$}%
\psfrag{007}[rc][rc]{\matlabtextA $44$}%
\psfrag{008}[rc][rc]{\matlabtextA $46$}%
\psfrag{009}[rc][rc]{\matlabtextA $48$}%
\psfrag{010}[rc][rc]{\matlabtextA $50$}%
\psfrag{011}[rc][rc]{\matlabtextA $52$}%
%
%% </ytick>

==> gfx/etrd_hexaHD_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{023}[cl][cl]{\matlabtextA data2}%
\psfrag{024}[cl][cl]{\matlabtextA dassssssta1}%
\psfrag{025}[bc][bc]{\matlabtextA PSNR}%
\psfrag{026}[tc][tc]{\matlabtextA Time}%
\psfrag{027}[bc][bc]{\matlabtextA PSNR}%
\psfrag{028}[tc][tc]{\matlabtextA Rate}%
%
%% </text>
%
%% <xscale>
%
\psfrag{012}[tc][tc]{\matlabtextA $\times10^{5}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $1000$}%
\psfrag{001}[ct][ct]{\matlabtextA $1200$}%
\psfrag{002}[ct][ct]{\matlabtextA $1400$}%
\psfrag{003}[ct][ct]{\matlabtextA $1600$}%
\psfrag{004}[ct][ct]{\matlabtextA $1800$}%
\psfrag{013}[ct][ct]{\matlabtextA $0$}%
\psfrag{014}[ct][ct]{\matlabtextA $5$}%
\psfrag{015}[ct][ct]{\matlabtextA $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextA $41$}%
\psfrag{006}[rc][rc]{\matlabtextA $42$}%
\psfrag{007}[rc][rc]{\matlabtextA $43$}%
\psfrag{008}[rc][rc]{\matlabtextA $44$}%
\psfrag{009}[rc][rc]{\matlabtextA $45$}%
\psfrag{010}[rc][rc]{\matlabtextA $46$}%
\psfrag{011}[rc][rc]{\matlabtextA $47$}%
\psfrag{016}[rc][rc]{\matlabtextA $40$}%
\psfrag{017}[rc][rc]{\matlabtextA $41$}%
\psfrag{018}[rc][rc]{\matlabtextA $42$}%
\psfrag{019}[rc][rc]{\matlabtextA $43$}%
\psfrag{020}[rc][rc]{\matlabtextA $44$}%
\psfrag{021}[rc][rc]{\matlabtextA $45$}%
\psfrag{022}[rc][rc]{\matlabtextA $46$}%
%
%% </ytick>

==> gfx/etrd_rect32_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextA data2}%
\psfrag{020}[cl][cl]{\matlabtextA dsssssssata1}%
\psfrag{021}[bc][bc]{\matlabtextA PSNR [dB]}%
\psfrag{022}[tc][tc]{\matlabtextA Encoding Times [s]}%
\psfrag{023}[bc][bc]{\matlabtextA PSNR [dB]}%
\psfrag{024}[tc][tc]{\matlabtextA File size [Bits]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0.98$}%
\psfrag{001}[ct][ct]{\matlabtextA $1$}%
\psfrag{002}[ct][ct]{\matlabtextA $1.02$}%
\psfrag{003}[ct][ct]{\matlabtextA $1.04$}%
\psfrag{004}[ct][ct]{\matlabtextA $1.06$}%
\psfrag{010}[ct][ct]{\matlabtextA $140$}%
\psfrag{011}[ct][ct]{\matlabtextA $160$}%
\psfrag{012}[ct][ct]{\matlabtextA $180$}%
\psfrag{013}[ct][ct]{\matlabtextA $200$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextA $55$}%
\psfrag{006}[rc][rc]{\matlabtextA $60$}%
\psfrag{007}[rc][rc]{\matlabtextA $65$}%
\psfrag{008}[rc][rc]{\matlabtextA $70$}%
\psfrag{009}[rc][rc]{\matlabtextA $75$}%
\psfrag{014}[rc][rc]{\matlabtextA $55$}%
\psfrag{015}[rc][rc]{\matlabtextA $60$}%
\psfrag{016}[rc][rc]{\matlabtextA $65$}%
\psfrag{017}[rc][rc]{\matlabtextA $70$}%
\psfrag{018}[rc][rc]{\matlabtextA $75$}%
%
%% </ytick>

==> gfx/hexa_stand_RD_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA data2}%
\psfrag{010}[cl][cl]{\matlabtextA ddfsdfsdfsdata1}%
\psfrag{011}[bc][bc]{\matlabtextA PSNR [dB]}%
\psfrag{012}[tc][tc]{\matlabtextA File size [Bits]}%
%
%% </text>
%
%% <xscale>
%
\psfrag{000}[tc][tc]{\matlabtextA $\times10^{5}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextA $0$}%
\psfrag{002}[ct][ct]{\matlabtextA $5$}%
\psfrag{003}[ct][ct]{\matlabtextA $10$}%
\psfrag{004}[ct][ct]{\matlabtextA $15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextA $40$}%
\psfrag{006}[rc][rc]{\matlabtextA $45$}%
\psfrag{007}[rc][rc]{\matlabtextA $50$}%
\psfrag{008}[rc][rc]{\matlabtextA $55$}%
%
%% </ytick>
